SycoPhantasy: Quantifying Sycophancy and Hallucination in Small Open Weight VLMs for Vision-Language Scoring of Fantasy Characters

Vision-language models (VLMs) are increasingly deployed as evaluators in tasks requiring nuanced image understanding, yet their reliability in scoring alignment between images and text descriptions remains underexplored. We investigate whether small, open-weight VLMs exhibit \emph{sycophantic} behavior when evaluating image-text alignment: assigning high scores without grounding their judgments in visual evidence. To quantify this phenomenon, we introduce the \emph{Bluffing Coefficient} (\bc), a metric that measures the mismatch between a model's score and its evidence recall. We evaluate six open-weight VLMs ranging from 450M to 8B parameters on a benchmark of 173,810 AI-generated character portraits paired with detailed textual descriptions. Our analysis reveals a significant inverse correlation between model size and sycophancy rate ($r = -0.96$, $p = 0.002$), with smaller models exhibiting substantially higher rates of unjustified high scores. The smallest model tested (LFM2-VL, 450M) produced sycophantic evaluations in 22.3\% of cases, compared to 6.0\% for the largest (LLaVA-1.6, 7B). These findings have direct implications for the deployment of small, open-weight VLMs as automated evaluators within attribute-rich, synthetic image evaluation tasks, where the gap between assigned scores and cited visual evidence is both measurable and consequential.

==> sections/experiments.tex <==
% =============================================================================
% EXPERIMENTS
% =============================================================================
% Lean experimental setup for main text; details in Appendix

\section{Experimental Setup}

This section describes the experimental configuration for our study. Full implementation details, including software dependencies and processing pipeline specifications, are provided in Appendix~\ref{sec:appendix_implementation}.

\subsection{Models and Inference}

We evaluate six open-weight VLMs spanning 450M to 8B parameters (Table~\ref{tab:models}). All models are instruction-tuned variants accessed via the Hugging Face Transformers library. We use greedy decoding to ensure deterministic, reproducible outputs. Models are loaded in bfloat16 precision and process images at 512$\times$512 resolution. Each model generates a JSON response containing the alignment score and reasoning, which we parse using robust extraction with fallback regex matching.

\subsection{Compute and Scale}

Experiments were conducted on NVIDIA A100 GPUs (40GB). Each model processes the full dataset of 173,810 image-description pairs, requiring approximately 8--20 hours depending on model size. Total compute across all six models was approximately 80 GPU-hours. All evaluation scripts support checkpointing for resumption from interruption.

\subsection{Analysis Configuration}

Our sycophancy analysis pipeline uses spaCy (en\_core\_web\_lg) for keyphrase extraction and BAAI/bge-large-en-v1.5 for semantic embedding. We apply a similarity threshold of $\tau = 0.75$ for keyphrase matching and a ROUGE-L threshold of 0.60 for parroting detection. Scores $\geq 70$ are classified as high, and scores $\leq 40$ as low, following the thresholds defined in Section~\ref{s}.

